A Framework for Fast and Stable Representations of Multiparameter Persistent Homology Decompositions

Topological data analysis (TDA) is an area of data science that focuses on using invariants from algebraic topology to provide multiscale shape descriptors for geometric data sets such as point clouds. One of the most important such descriptors is {\em persistent homology}, which encodes the change in shape as a filtration parameter changes; a typical parameter is the feature scale. For many data sets, it is useful to simultaneously vary multiple filtration parameters, for example feature scale and density. While the theoretical properties of single parameter persistent homology are well understood, less is known about the multiparameter case. In particular, a central question is the problem of representing multiparameter persistent homology by elements of a vector space for integration with standard machine learning algorithms. Existing approaches to this problem either ignore most of the multiparameter information to reduce to the one-parameter case or are heuristic and potentially unstable in the face of noise. In this article, we introduce a new general representation framework that leverages recent results on {\em decompositions} of multiparameter persistent homology. This framework is rich in information, fast to compute, and encompasses previous approaches. Moreover, we establish theoretical stability guarantees under this framework as well as efficient algorithms for practical computation, making this framework an applicable and versatile tool for analyzing geometric and point cloud data. We validate our stability results and algorithms with numerical experiments that demonstrate statistical convergence, prediction accuracy, and fast running times on several real data sets.

==> macros.tex <==
% Definitions of handy macros can go here

\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand\CC{C\nolinebreak\hspace{-.05em}\raisebox{.4ex}{\relsize{-3}{\textbf{+}}}\nolinebreak\hspace{-.10em}\raisebox{.4ex}{\relsize{-3}{\textbf{+}}}}

% Maths shortcuts
\newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\Esub}[2]{\mathbb{E}_{#2} \left[ #1 \right]}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\scalar}[1]{\left\langle #1 \right\rangle}
\newcommand{\X}{\mathcal{X}}
\newcommand{\ind}[1]{\mathds{1}_{\{#1\}}}
\newcommand{\pairing}{{\rm Low}}
\newcommand{\reduced}{{\rm bd}}
\newcommand{\swap}{{\rm sw}}
\newcommand{\disti}{{d_I}}
\newcommand{\distb}{{d_b}}
\newcommand{\fibered}[1]{ {\mathcal F}{\mathcal B}(#1) }
\newcommand{\barcode}[1]{ {\mathcal B}(#1) }
\newcommand{\conv}[1]{ {\rm conv}(#1) }
\newcommand{\dir}[1]{ {\rm dir}(#1) }
\newcommand{\codir}[1]{ {\rm codir}(#1) }
\newcommand{\induced}[1]{\mathrm{ \mathbf{ Ind}}\left(#1\right) }
\DeclareRobustCommand*{\ora}{\overrightarrow}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\e}{{\bf e}}
\newcommand{\uv}{{\bf u}}
\newcommand{\M}{{\mathbb M}}
\newcommand{\di}{d_{\rm I}}
\newcommand{\db}{d_{\rm B}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\bdelta}{\boldsymbol \delta}


\newcommand{\dgm}{\mathrm{dgm}}
\newcommand{\pop}{\mathrm{op}}
\newcommand{\repr}{V}
\newcommand{\bars}{\mathrm{bcd}}
\newcommand{\bottleneck}{\mathrm{d}_B}
\newcommand{\malpha}{\mathrm{a}}
\newcommand{\vine}{\mathrm{vine}}
\newcommand{\match}{\mathrm{m}}
\newcommand{\fell}{f_{\ell}}
\newcommand{\fells}[1]{f_{\ell_{#1}}}

\newcommand{\field}{k}
\newcommand{\upperb}[1]{ U[#1] }
\newcommand{\lowerb}[1]{ L[#1] }
\newcommand{\birthcp}[1]{ C_B(#1) }
\newcommand{\deathcp}[1]{ C_D(#1) }
\newcommand{\birthLcp}[1]{ C_B^L(#1) }
\newcommand{\deathLcp}[1]{ C_D^L(#1) }
\newcommand{\supp}[1]{ {\rm supp}\left(#1\right) }
\newcommand{\dd}{\, \mathrm d}
% \newcommand{\supp}[1]{ {\rm supp}(#1) }
\newcommand{\rectangle}[2]{ R_{#1, #2} }
\newcommand{\interior}[1]{%
  {\kern0pt#1}^{\mathrm{o}}%
}
\newcommand\restr[2]{{   %%% Restriction of a set
  \left.\kern-\nulldelimiterspace 
  #1 
  \vphantom{\big|}
  \right|_{#2}
  }}

\newcommand{\RIVET}{\texttt{Rivet}}

\newcommand{\bound}{}
\newcommand{\twobound}{2}

\SetKwComment{Comment}{/* }{ */}
\newcommand{\ms}{\texttt{ms}}

%%%% Theorems, props
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\newtheorem{example}[theorem]{Example}


==> packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage[left=2cm,right=2cm,top=2cm,bottom=2cm]{geometry} % marges
\usepackage{hyperref}       % hyperlinks
\usepackage{amsmath,amsfonts,amsthm}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{stmaryrd}
\usepackage{pst-node}
\usepackage{tikz-cd}
\usepackage{dsfont}             %pourindicator functions
\usepackage{tipa}
\usepackage{tikz}
\usetikzlibrary{cd}
\usepackage{algorithm2e}
\RestyleAlgo{ruled}
\usepackage{todo}
\usepackage{verbatim}
\usepackage{subcaption}
%\usepackage{algorithm}
\usepackage{algpseudocode}
%%%%%%%% subfiles 
\usepackage{import}


%%%%% FONTS
\usepackage{libertine}%\usepackage[ttscale=.875]{libertine}
\renewcommand*{\ttdefault}{lmvtt} % ou autre police monospace
\usepackage[libertine]{newtxmath}
%%%%%%% SECTIONS STYLE
\usepackage{titlesec}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}}

\titlelabel{\thetitle. }
\titleformat{\section}{\center\large\bfseries\boldmath}{\thesection.}{1ex}{}
\titleformat{\subsection}{\center\bfseries\boldmath}{\thesubsection.}{1ex}{}

\newcommand{\periodafter}[1]{\ifstrempty{#1}{}{#1.}}
\titleformat{\subsubsection}[runin]{\bfseries\boldmath}{\thesubsubsection.}{1ex}
{\periodafter}


%%%% IMAGE STUFF
\usepackage{graphics}
\usepackage{svg,float}
\usepackage{graphicx}
